Connecting the Dots: Evaluating Abstract Reasoning Capabilities of LLMs Using the New York Times Connections Word Game

The New York Times Connections game has emerged as a popular and challenging pursuit for word puzzle enthusiasts. We collect 438 Connections games to evaluate the performance of state-of-the-art large language models (LLMs) against expert and novice human players. Our results show that even the best performing LLM, Claude 3.5 Sonnet, which has otherwise shown impressive reasoning abilities on a wide variety of benchmarks, can only fully solve 18% of the games. Novice and expert players perform better than Claude 3.5 Sonnet, with expert human players significantly outperforming it. We create a taxonomy of the knowledge types required to successfully cluster and categorize words in the Connections game. We find that while LLMs perform relatively well on categorizing words based on semantic relations they struggle with other types of knowledge such as Encyclopedic Knowledge, Multiword Expressions or knowledge that combines both Word Form and Meaning. Our results establish the New York Times Connections game as a challenging benchmark for evaluating abstract reasoning capabilities in AI systems.

==> garbage.tex <==
% \begin{table*}[!ht]
% \renewcommand{\arraystretch}{1.35}
% \centering
% \small
% \begin{tabular}{|ll|l|l|}
% \hline

% \multicolumn{2}{|l|}{\textbf{Knowledge}}                             & \textbf{Category}                         & \textbf{Words}                                          \\ \hline
% \multicolumn{2}{|l|}{\multirow{2}{*}{Encyclopedic}}         & \begin{tabular}[c]{@{}l@{}}TV SHOWS WITH \\ HAPPY-SOUNDING NAMES\end{tabular} & {[}`CHEERS', `EUPHORIA', `FELICITY', `GLEE'{]} \\ \cline{3-4} 
% \multicolumn{2}{|l|}{}                                      & JACKS                 & {[}`BLACK', `FROST', `MA', `SPARROW'{]}       \\ \hline\hline
% \multicolumn{1}{|l|}{\multirow{3}{*}{Semantic}}  & Synonym  & COLLEAGUES                         & {[}`ASSOCIATE', `FELLOW', `PARTNER', `PEER'{]} \\ \cline{2-4} 
% \multicolumn{1}{|l|}{}                           & Polysemy & WHAT A MOLE CAN BE                 & {[}`ANIMAL', `BIRTHMARK', `SPY', `UNIT'{]}     \\ \cline{2-4} 
% \multicolumn{1}{|l|}{}                           & Hypernym & PERIOD                             & {[}`AGE', `DAY', `ERA', `TIME'{]}              \\ \hline\hline
% \multicolumn{2}{|l|}{\multirow{2}{*}{Associative}}          &  ORIGIN           & {[}`CRADLE', `FONT', `ROOT', `SOURCE'{]}    \\ \cline{3-4} 
% \multicolumn{2}{|l|}{}                                      & THINGS THAT ARE ORANGE            & {[}`BASKETBALL', `CARROT', `GOLDFISH', `PUMPKIN'{]}     \\ \hline\hline
% \multicolumn{2}{|l|}{\multirow{2}{*}{Linguistic}}           & NOUN SUFFIXES                      & {[}`DOM', `ION', `NESS', `SHIP'{]}             \\ \cline{3-4} 
% \multicolumn{2}{|l|}{}                                      & SILENT ``W"               & {[}`ANSWER', `TWO', `WRIST', `WRONG'{]}        \\ \hline\hline
% \multicolumn{2}{|l|}{\multirow{1}{*}{Multiword Expression}} & \_\_\_WOOD                         & {[}`DOG', `DRIFT', `HOLLY', `SANDAL'{]}        \\
% % \multicolumn{2}{|l|}{}                                      & SECRET \_\_\_                      & {[}`AGENT', `CODE', `SANTA', `SAUCE'{]} 
% \hline\hline
% \multicolumn{2}{|l|}{\multirow{2}{*}{Combined}} & CITY HOMOPHONES                         & {[}`DELI', `NIECE', `ROAM', `SOUL'{]}        \\ \cline{3-4} 
% \multicolumn{2}{|l|}{}                                      & SOCIAL MEDIA APP ENDINGS                      & {[}`BOOK', `GRAM', `IN', `TUBE'{]}        \\ \hline
% \end{tabular}
% \caption{\label{knowledgetype}Different types of knowledge required to group words into their respective categories}
% \end{table*}

% \begin{table*}[!ht]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \begin{tabular}[c]{@{}c@{}}\textbf{Semantic} \\ \textbf{Knowledge}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Associative} \\ \textbf{Knowledge}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Encyclopedic} \\ \textbf{Knowledge}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Mutiword} \\ \textbf{Expressions}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Linguistic} \\ \textbf{Knowledge}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Combined} \\ \textbf{Knowledge}\end{tabular} \\ \hline
% 337 & 171 & 153 & 77 & 49 & 13 \\ \hline
% \end{tabular}
% \caption{\label{reasoningbreakdown}Breakdown of instances of different types of reasoning across 800 categories from 200 Connections games}
% \end{table*}

% Investigating the relationship between words offers insights into both the structure of language and the influence of cognition on linguistic tasks \cite{stella2018multiplex}. To solve Connections games, players must draw on certain aspects of word knowledge, such as a word’s meaning. To deepen our understanding, we bucket each $<$category, grouping$>$ into the types of knowledge that are primarily required to solve them. Two experts annotate a total of 800 samples coming from 200 games into 6 broader categories. On 8.6\% of the 800 samples where they disagree (See examples of disagreement in Appendix \ref{appendix:disagree}), the experts engaged in discussion \cite{10.1145/3274423,10.1145/3610074,10.1145/3290605.3300761} to arrive at an individual category.

\subsubsection{Multiword Expressions} Multiword Expressions are complex constructs that interact in various, often untidy ways and represent a broad continuum between non-compositional (or idiomatic) and compositional groups of words \cite{moon1998fixed}. Higher difficulty levels (blue and purple) in the Connections game often require players to recognize that the four words can form a Multiword Expression if combined with an external word. Table \ref{knowledgetype} shows examples of Multiword Expressions where half of the expressions are given in the form of individual words and the player needs to find the other half to categorize words into the correct group. 

\subsubsection{Linguistic Knowledge} Linguistic competence \cite{coseriu1985linguistic} is the system of unconscious knowledge that one has when one knows a language. Such competence is often required to classify words into their appropriate categories. Several instances from the Connections game require knowledge of morphology, phonology, or orthography for correct categorization. For example, as shown in Table \ref{knowledgetype}, one needs knowledge about morphology to group \emph{Dom, Ion, Ness,} and \emph{Ship} as \emph{Noun Suffixes}. Similarly, one needs to rely on phonological knowledge about the sound patterns of \emph{Answer, Two, Wrist,} and \emph{Wrong} to categorize them as \emph{Silent "W"}.

==> latex/dump.tex <==
% \begin{itemize}
% \item Number of total answers: 3028
%     \begin{itemize}
%     \item Number of unique answers: 2200 ($\sim$72.655\% of the total answers)
%     \end{itemize}

% \item Number of categories: 1084
% \begin{itemize}
%         \item Number of unique categories: 993 ($\sim$91.605\% of the total categories)
%     \end{itemize}
% \end{itemize}

% The full dataset and code used to scrape and analyze the data can be found at the following address: \href{https://github.com/mustafamariam/LLM-Connections-Solver}{https://github.com/mustafamariam/LLM-Connections-Solver}. 


% \subsection{Data Analysis} \label{sec:data_analysis}
% An analysis of the collected NYT Connections answers reveals potential problem-solving difficulties and trends.

% \subsubsection{Repetition}
% In total, 828 answer words, or $\sim$27.345\% were repeated. The most common words and their respective frequencies are RING (8) and WING (8). Many words repeat more than twice. In contrast, only 42 or $\sim$8.395\% categories were repeated. The most common category was HOMOPHONES (5). Most repeating categories are repeated only twice.

% This analysis suggests oftentimes, the same word is used in different categories. The LLM will have to understand multiple senses of a word and decide which one works best in the classification context.

% \subsubsection{Clustering}
% We performed an initial KMeans clustering on the data after using the silhouette score algorithm to find the optimal cluster amount. After cleaning, we produced the following 9 clusters:
% \begin{enumerate}
% \item Cluster 1: Fill in the Blank
% \begin{itemize}
% \item Size = 91
% \item Examples: \_\_\_ DREAM, LIVING \_\_\_, BELLY \_\_\_ (\_\_\_ indicates a blank that the answer word must fill.)
% \end{itemize}
% \item Cluster 2: Things That/With
% \begin{itemize}
% \item Size = 36
% \item Examples: THINGS WITH SPINES, THINGS MADE WITH FEATHERS, THINGS THAT WHISTLE
% \end{itemize}
% \item Cluster 3: Words Starting/Ending/Containing
% \begin{itemize}
% \item Size = 24
% \item Examples: WORDS ENDING IN CLOTHING, WORDS BEGINNING WITH INSTRUMENTS, WORDS WITH THREE G'S
% \end{itemize}
% \item Cluster 4: Parts-Related
% \begin{itemize}
% \item Size = 22
% \item Examples: PARTS OF AN AIRPORT, PARTS OF FRUIT YOU MIGHT NOT EAT, PARTS OF A DOOR
% \end{itemize}
% \item Cluster 5: Animal-Related
% \begin{itemize}
% \item Size = 13
% \item Examples: ANIMALS BACKWARD, MALE ANIMALS, BLACK-AND-WHITE ANIMALS
% \end{itemize}
% \item Cluster 6: Names-Related (Proper Nouns)
% \begin{itemize}
% \item Size = 11
% \item Examples: CLASSIC DOG NAMES, NEWSPAPER NAMES, ROAD NAMES
% \end{itemize}
% \item Cluster 7: Homophones
% \begin{itemize}
% \item Size = 8
% \item Examples: VEGETABLE HOMOPHONES, CITY HOMOPHONES, COLOR HOMOPHONES
% \end{itemize}
% \item Cluster 8: What X Might Mean
% \begin{itemize}
% \item Size = 7
% \item Examples: WHAT “K” MIGHT MEAN, WHAT “BLUE” MIGHT MEAN, WHAT “O” MIGHT MEAN
% \end{itemize}
% \item Cluster 9: Food-Related
% \begin{itemize}
% \item Size: = 6
% \item Examples: WAYS TO PRESERVE FOOD, TORUS-SHAPED FOOD, WAYS TO GATHER FOOD
% \end{itemize}
% \end{enumerate}
% The clustering results primarily display the difficulty of the solving task. Notably, we removed one miscellaneous cluster with a size of 736, indicating that a large number of categories were difficult to cleanly classify. The categories also cover many relevant areas in NLP -- including semantics, structure, named entity recognition, and cultural context -- which relate to the type of reasoning the LLM will have to employ to solve this task.


% This information is stored in what cognitive scientists call our semantic memory \cite{quillian1966semantic}. On the contrary, word knowledge is also typically structured through associative learning, which occurs when an element is taught through association with another separate, pre-occurring element \cite{shanks1995psychology}. The Connections games also frequently require possessing domain-specific encyclopedic knowledge \footnote{\url{https://en.wikipedia.org/wiki/Encyclopedic_knowledge}} to make connections between certain words. Last but not least, to successfully solve the Connections game, one needs knowledge about Multiword expressions and Linguistic Knowledge (e.g., Orthography, Morphology etc). 

% \begin{itemize}
% \item $w_0 = 1 $ for Yellow (level 1; most straightforward) correct grouping
% \item $w_1 = 2 $ for Green (level 2) correct grouping
% \item $w_2 = 3 $ for Blue (level 3) correct grouping
% \item $w_3 = 4 $ for Purple (level 4; trickiest) correct grouping
% \end{itemize}
% A player will only be rewarded based on the categories they get correct; a higher difficulty of grouping deserves to be assigned a greater weight and overall score. The minimum score a player can receive is 0 (no classifications correct), while the greatest overall score a player can receive is 10.

% \begin{figure*}[!ht]
%     \small
%     \centering
%     \includegraphics[width=1.0\textwidth]{pictures/weighted_classification.png}
%     \caption{Weighted classification score according to scoring schema in Sections~\ref{sec:scoring} for each model across 200 Connections games}
%     \label{fig:weighted_score}
% \end{figure*}

%Lexical items participate in regular patterns of association with each other. %SM-new you say association so it is not clear why is not associative then and is semantic
%Some relations between lexical items include \emph{synonyms} (similarities), \emph{hypernyms/hyponyms} (hierarchical structures), and \emph{polysemy} (many possible meanings for a word). 
%We find a lot of such relations covered in the Connections game. 

Examples of Multiword Expressions correctly classified by Claude3-Opus but no other model include:
\begin{enumerate}
    \item \_\_\_ BERRY: ['BLUE', 'GOOSE', 'RASP', 'STRAW']
    \item \_\_\_ PAPER: ['BUTCHER', 'SCRAP', 'TOILET', 'WAX']
\end{enumerate}

% Since humans did not have to provide reasoning for their classifications, we measured their reasoning abilities simply through the groups they classified correctly.

Researchers have been investigating the ability of LLMs to engage in various aspects of gaming, showcasing their versatility. Studies have shown that these models can serve as competent players, taking on the role of human participants in different game scenarios \cite{wang2023voyager, tsai2023can, ciolino2020go, meta2022human, noever2020chess}. Additionally, LLMs have demonstrated the capacity to act as non-player characters (NPCs), enriching the gaming experience by providing intelligent and interactive characters within the game world \cite{park2023generative,urbanek2019learning}. Furthermore, these models have exhibited promise in generating game content, such as creating novel game assets, storylines, and environments \cite{todd2023level,wang-etal-2023-bytesized32,sudhakaran2024mariogpt,ammanabrolu2021modeling}

